Decomposing Generalization: Models of Generic, Habitual, and Episodic Statements

We present a novel semantic framework for modeling linguistic expressions of generalization---generic, habitual, and episodic statements---as combinations of simple, real-valued referential properties of predicates and their arguments. We use this framework to construct a dataset covering the entirety of the Universal Dependencies English Web Treebank. We use this dataset to probe the efficacy of type-level and token-level information---including hand-engineered features and static (GloVe) and contextual (ELMo) word embeddings---for predicting expressions of generalization. Data and code are available at decomp.io.

==> tables/spr_arg.tex <==
\setlength\tabcolsep{4pt}
\begin{tabular}{lrrr}
\toprule
\textbf{Property} & \textbf{Is Part} & \textbf{Is Kind} & \textbf{Is Abs} \\
\midrule
awareness & 0.16 & -0.1 & -0.15 \\
volition & 0.16 & -0.11 & -0.15 \\
sentient & 0.16 & -0.08 & -0.16 \\
instigation & 0.10 & -0.08 & -0.09 \\
existed before & 0.16 & -0.04 & -0.17 \\
existed during & 0.10 & -0.02 & -0.07 \\
existed after & 0.15 & -0.06 & -0.14 \\
was for benefit & 0.11 & -0.08 & -0.11 \\
change of location & 0.07 & 0.06 & -0.17 \\
change of state & -0.02 & 0.03 & -0.03 \\
was used & 0.08 & -0.03 & -0.09 \\
change of possession & -0.04 & 0.11 & -0.04 \\
partitive & -0.02 & 0.04 & -0.06 \\
\bottomrule
\end{tabular}

